Explainable Multivariate Time Series Classification: A Deep Neural Network Which Learns To Attend To Important Variables As Well As Informative Time Intervals

Time series data is prevalent in a wide variety of real-world applications and it calls for trustworthy and explainable models for people to understand and fully trust decisions made by AI solutions. We consider the problem of building explainable classifiers from multi-variate time series data. A key criterion to understand such predictive models involves elucidating and quantifying the contribution of time varying input variables to the classification. Hence, we introduce a novel, modular, convolution-based feature extraction and attention mechanism that simultaneously identifies the variables as well as time intervals which determine the classifier output. We present results of extensive experiments with several benchmark data sets that show that the proposed method outperforms the state-of-the-art baseline methods on multi-variate time series classification task. The results of our case studies demonstrate that the variables and time intervals identified by the proposed method make sense relative to available domain knowledge.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> proposed_backup.tex <==
\section{Attention CNN}
\subsection{Notations}
In this subsection, we first define some notations that will be used throughout the paper unless otherwise noted. We denote a multi-variable time series sequence by $\mathbf{X} = \left\lbrace \mathbf{x}^{(1)},\ldots,\mathbf{x}^{(T)} \right\rbrace$, where $\mathbf{x}^{(t)} \in \R^P$ denotes the $P$ dimensional observation at time point $t$. We use $\mathbf{x}^{(t)}_i \in \R$ to denote the value of the $i$-th variable sampled at time point $t$. A set of input sequences along with their true labels are denoted by $\left\lbrace (\mathbf{X}_1,y_1),\ldots,(\mathbf{X}_N,y_N) \right\rbrace$. Based on the context, $t$ can be used to index either a time point or a time interval.
\subsection{Problem Definition\aaron{not done yet}}
In this study, we focus on predicting the class label of multi-variable time series data with an interpretable model.





problem 0: multi-variate time series classification

problem 1: locality awareness

problem 2: interpretable reasoning


\subsection{Model}
% Against this background, the proposed model aims at providing interpretable decision making by identifying informative time series features and the time intervals of interest (TOI) in a time series classification task.

% We propose feature and temporal convolutional attention time series (FAT-CAT) learning model for interpretable multi-variable time series classification task and a sketch of the model is depicted in Figure~\ref{fig:FATCAT_flowchart}. The model mainly consists of three components, convolutional layer feature extraction, variable-wise attention score evaluation, and temporal-wise attention score evaluation.

The key idea of FAT-CAT is to construct a summary embedding from the multi-variate time series sequence by exploiting convolutional layer to enable local information extraction and adopting two attention measure evaluation modules to identify informative time segments and variables. The well-learned summary embedding would contain key information that allows accurate downstream classification task. In essence, the model can be formulated as
\begin{equation}
    \label{eq:prob_model}
    p(y\vert \mathbf{X}) = p(\mathbf{z} \vert \mathbf{X}) \cdot p(y\vert \mathbf{z})
\end{equation}
where $\mathbf{z}$ is the summary embedding. In the joint distribution, the first part focus on extracting key information from the input sequence and the second part aims at making accurate prediction. A sketch of the model framework is depicted in Figure~\ref{fig:FATCAT_flowchart}. We begin with discussing the first part, composing informative summary embedding.

\begin{figure*}[t]
    \centering
    \includegraphics[width = 0.96\textwidth]{flowchart.png}
    \caption{\aaron{refine figure}}
    \label{fig:FATCAT_flowchart}
\end{figure*}

\subsubsection{Convolutional Layer Feature Extraction}
The key idea of the feature extraction level is to incorporate local context as opposed to focus only on point-wise observations. Given a multi-variable time series input sequence $\mathbf{X} = \left\lbrace \mathbf{x}^{(1)}, \ldots, \mathbf{x}^{(T)} \right\rbrace$, with $\mathbf{x}^{(t)} \in \R^P$, where $T$ is the length of the sequence and $P$ is the number of covariates, we adopt convolutional layer to automatically extract features from raw sequences.

Specifically, a $1-d$ convolutional layer with kernel size $1 \times L$ is applied on each input sequence where $L$ is the length of the time interval of interest. The kernel window slides through the temporal domain with overlap. The convolutional weight is shared along the temporal domain and each input variable has its own dedicated feature extraction convolutional layer. In our model, we adopt a convolutional layer with $J$ filters so that a $J$-dimensional feature vector is extracted for each input sequence from every time interval. In essence, the convolutional layer encodes multi-variable input sequence as follows \aaron{elaborate more}
\begin{equation}
    \label{eq:cnn_feature_extraction}
    \left\lbrace \mathbf{c}_{i,t} \right\rbrace = CNN_i\left( \mathbf{x}_i \right)
\end{equation}
where $\mathbf{c}_{i,t} \in \R^J$ is the feature vector for variable $\mathbf{x}_i$ extracted from the $t$-th time interval of interest, $i=1,\ldots,P$ and $t=1,\ldots,l$. Note that $l$, number of intervals, depends on the window length $L$ and the overlap. The encoding obtained from such extraction preserves local information while the filters attend to different aspects of the input sequence. In addition, the length of the sequence is significantly reduced by considering intervals instead of time points. Hence, the computational complexity for downstream attention evaluation is reduced drastically. We leave the exploration of exploiting advanced convolutional structures as promising future direction. For example, incorporating dilated convolution~\cite{oord2016wavenet} for more flexible receptive field.

\subsubsection{Dual Attention}
After sending an input sequence $\left\lbrace \mathbf{x}_1, \ldots, \mathbf{x}_T \right\rbrace$ into the convolutional feature extraction layer, we obtain a sequence of feature matrices $\left\lbrace \mathbf{C}_1,\ldots,\mathbf{C}_{l} \right\rbrace$, where $\mathbf{C}_t \in \R^{P\times J}$. Each row in $\mathbf{C}_t$ stores the feature vector specific to each variable within time interval $t$ in the input sequence.

The mechanism of the dual attention begins with considering the feature matrices at each time interval so as to obtain a local context embedding vector $\mathbf{h}_t, t=1,\ldots,l$, for each interval. Thereafter, temporal attention is derived from the context embedding vectors and exploited to construct the final summary embedding $\mathbf{z}$, which is then used for downstream task. The two attention modules can be formulated in a probabilistic mixture model as
\begin{equation}
    \label{eq:att_prob_model}
    \begin{aligned}
        p( \mathbf{z} \vert \mathbf{X})
        &= \sum_{t=1}^{l} p( \mathbf{z} \vert u = t, \mathbf{X}) p( u=t \vert \mathbf{X})\\
        &= \sum_{t=1}^{l} p(\mathbf{z} \vert u = t, \mathbf{h}_t) p(u=t \vert \mathbf{h}_1,\ldots, \mathbf{h}_{l}) p(\mathbf{h}_t \vert \mathbf{X})\\
        &= \sum_{t=1}^{l} p(\mathbf{z}\vert u = t,\mathbf{h}_t)p(u=t \vert \mathbf{h}_1,\ldots, \mathbf{h}_{l})\\
        &\hspace{0.25cm} \cdot \left( \sum_{i=1}^P p(\mathbf{h}_t \vert v_t=i, \mathbf{X})p(v_t=i \vert \mathbf{X})  \right)\\
        &= \sum_{t=1}^{l} p(\mathbf{z}\vert u = t,\mathbf{h}_t) \underbrace{p(u=t \vert \mathbf{h}_1,\ldots, \mathbf{h}_{l})}_{\text{temporal attn.}}\\
        &\hspace{0.25cm} \cdot \left( \sum_{i=1}^P p(\mathbf{h}_t \vert v_t=i, \mathbf{c}_{i,t}) \underbrace{p(v_t=i \vert \mathbf{C}_t)}_{\text{variable attn.}}  \right)
    \end{aligned}
\end{equation}
In the above formulation, we introduce auxiliary variables $u$ and $v_t$ in to the density function. The variable $u$ is a discrete variable taking values on the index of the time intervals, i.e. on the set $\left\lbrace 1,\ldots,l \right\rbrace$. The variable $v_t$ refers to the input variables at the $t$-th time interval and takes values over the set $\left\lbrace 1,\ldots,P \right\rbrace$. In the model, $p(u=t \vert \mathbf{h}_1,\ldots, \mathbf{h}_{l})$ controls the contribution of each time interval to the construction of the summary embedding while $p(v_t=i \vert \mathbf{C}_t)$ controls the extent to which variable $i$ dominates interval $t$. The following subsections discuss the attention modules used to evaluate these densities.

\subsubsection{Learning Local Context Embedding by Variable Attention}
The first attention module evaluates variable attention and constructs local context embedding. Without loss of generality, we model $p(v_t = i \vert \mathbf{C}_t)$ with a Gaussian distribution $\mathcal{N}(\alpha_{i_t},\sigma_{i_t})$, and $\mathbf{a}_t = \left[ \alpha_{1_t}, \ldots, \alpha_{P_t} \right]$ is obtained by the variable attention scoring function characterized by the following
\begin{equation}
    \label{eq:feature_attention}
    \begin{aligned}
        &\mathbf{a}_t = softmax \left( \mathbf{s}_t \right)\\
        &\mathbf{s}_t = \sigma_2 \left( \sigma_1 \left( W_1^{\left( V \right)} \mathbf{C}_t + B_1^{\left( V \right)} \right)W_2^{\left( V \right)} + B_2^{\left( V \right)} \right)
    \end{aligned}
\end{equation}
where $W_1^{\left( V \right)} \in \R^{1 \times P}$, $W_2^{\left( V \right)} \in \R^{J \times P}$, $B_1^{\left( V \right)} \in \R^{1 \times J}$, $B_2^{\left( V \right)} \in \R^{1 \times P}$ are the model parameters, and $\sigma_1 \left( \cdot \right)$, $\sigma_2 \left( \cdot \right)$ are non-linear activation functions, for example tanh, ReLU among others.

Next, we proceed to construct the local context embedding with the variable attention score. For the distribution $p(\mathbf{h}_t \vert v_t=i, \mathbf{c}_{i,t})$, we have $\mathbf{h}_t = \mathbf{c}_{i,t}$ with probability one. The reasons for the simple procedure are twofold: 1) the attention scores are evaluated upon $\mathbf{c}_{i,t}$ and thus should be weighted directly on it; 2) for the sake of computation efficiency. In conclusion the distribution of the local context embedding $p(\mathbf{h}_t \vert \mathbf{X})$ is a Gaussian distribution with the mean given by
\begin{equation}
    \label{eq:context_vector_time}
    \mathbf{h}_t = \sum_{i=1}^P \alpha_{i_t}\mathbf{c}_{i,t}
\end{equation}
with a slight abuse of notation.

To this stage, we have obtained the local context embeddings for all the time intervals by considering the relative variable importance. Note that the constructions of the local context embeddings are independent to each other and hence need not to be processed in a sequential order. In addition, the variable attention scoring function is shared among all intervals to be efficient on the amount of model parameters.

\subsubsection{Learning Final Summary Vector by Temporal Attention}
When the second stage is completed, we obtain a context matrix $\mathbf{H} = \left[ \mathbf{h}_1^T, \ldots, \mathbf{h}_{l}^T \right]^T \in \R^{l \times J}$ consisting of the context vectors constructed by taking into account the importance of each individual variable. In the next step, we compose the summary embedding with temporal importance by the temporal attention module.

Similarly, $p(u=t \vert \mathbf{h}_1,\ldots, \mathbf{h}_{l})$ is modelled by a Gaussian distribution without loss of generality. The Gaussian distribution is parameterized by $\mathcal{N}(\beta_t,\delta_t)$ and $\mathbf{b} = \left[ \beta_1, \ldots, \beta_{l} \right]$ is measured by the temporal attention module characterized by
\begin{equation}
    \label{eq:temporal_attention}
    \begin{aligned}
        &\mathbf{b} = softmax \left( \mathbf{u} \right)\\
        &\mathbf{u} = \sigma_2 \left( \sigma_1 \left( W_1^{\left( T \right)} \mathbf{H} + B_1^{\left( T \right)} \right)W_2^{\left( T \right)} + B_2^{\left( T \right)} \right)
    \end{aligned}
\end{equation}
where $W_1^{\left( T \right)} \in \R^{1 \times l}$, $W_2^{\left( T \right)} \in \R^{J \times l}$, $B_1^{\left( T \right)} \in \R^{1 \times J}$, and $B_2^{\left( T \right)} \in \R^{1 \times l}$ are model parameters, and $\sigma_1 \left( \cdot \right)$, $\sigma_2 \left( \cdot \right)$ are non-linear activation functions. The temporal attention scores are then used to compose the final summary vector. Based on the aforementioned argument, for $p(\mathbf{z} \vert u = t, \mathbf{h}_t)$, we have $\mathbf{z} = \mathbf{h}_t$ definitely. Hence, we arrive at the conclusion that the summary vector $\mathbf{z}$ is given by
\begin{equation}
    \label{eq:summary_vector}
    \mathbf{z} = \sum_{t=1}^{l} \beta_t \mathbf{h}_t
\end{equation}
This concludes the first part, extracting key information from the multi-variable input sequence.

\subsubsection{Classifying The Input Sequence}
In the second part, the obtained summary vector is used to predict the label. The distribution $p(y \vert \mathbf{z})$ is derived by a nonlinear function $f(\mathbf{z})$, where $f(\cdot)$ can be a feed forward neural network. Though we focus on predicting the label of the input sequence, one can design appropriate function based on different tasks. For example the framework can also be applied on forecasting task by replacing an appropriate regression function. This unified framework simultaneously predicts the label of the input sequence and provides insights to the decision making.

\subsection{Learning and Interpreting The Model}
Given a set of training instances $\left\lbrace (\mathbf{X}_1,y_1),\ldots,(\mathbf{X}_N,y_N) \right\rbrace$, the model parameters $\Theta$ are found by optimizing the objective function
\begin{equation}
    \label{eq:model_obj}
    \sum_{i=1}^N \mathcal{L}(\mathbf{X}_i, y_i; \Theta)
\end{equation}
In this study, the proposed model is applied on time series classification task and is learned to minimize the cross entropy loss function. The model is smooth and differentiable and therefore can be optimized by standard gradient back propagation. We exploited the Adam optimizer~\cite{kingma2014adam} to train the model parameters where the hyperparameters of the Adam optimizer is set to its default values.
% \subsection{Interpreting The Model}

The capability of providing interpretable reasoning is essential for a machine learning model nowadays in addition to giving accurate predictions. The proposed model aims not only at accurate classification of multi-variable time series data but also at identifying the key time intervals and variables that contributes to the final decision making without the need of extensive post analyzing. After the training process is completed, we can extract three results from the model given a data instance, namely label prediction, temporal attention score, and variable attention score. As depicted in Figure~\ref{fig:interpret_att}, to interpret the result, the temporal attention score vector $\mathbf{b}$ measures the contribution of each time interval. By removing the irrelevant ones, we focus only on the informative time segments. Within that, one can further refer to the variable attention score vectors $\mathbf{a}_t$ so as to find the key variables within the selected segments. With only light post analysis, the two attention modules combined provide instance-specific temporal and variable selection. These results can then be verified by domain knowledge or guide domain research.

\begin{figure}
    \centering
    \includegraphics[width = 0.4\textwidth]{flowchart2.png}
    \caption{Caption}
    \label{fig:interpret_att}
\end{figure}

%  The size of mini-batch is set to 40. The model is implemented in the PyTorch framework~\cite{paszke2019pytorch}.
